PTQ4ViT: Post-training quantization for vision transformers with twin uniform quantization

Quantization is one of the most effective methods to compress neural networks, which has achieved great success on convolutional neural networks (CNNs). Recently, vision transformers have demonstrated great potential in computer vision. However, previous post-training quantization methods performed not well on vision transformer, resulting in more than 1% accuracy drop even in 8-bit quantization. Therefore, we analyze the problems of quantization on vision transformers. We observe the distributions of activation values after softmax and GELU functions are quite different from the Gaussian distribution. We also observe that common quantization metrics, such as MSE and cosine distance, are inaccurate to determine the optimal scaling factor. In this paper, we propose the twin uniform quantization method to reduce the quantization error on these activation values. And we propose to use a Hessian guided metric to evaluate different scaling factors, which improves the accuracy of calibration at a small cost. To enable the fast quantization of vision transformers, we develop an efficient framework, PTQ4ViT. Experiments show the quantized vision transformers achieve near-lossless prediction accuracy (less than 0.5% drop at 8-bit quantization) on the ImageNet classification task.

==> 5_discussion.tex <==
\section{Discussion}

% In this section, we will discuss the inference efficiency of the twin quantization format on hardware devices.
% Then we will discuss the number of calibration images and the quantization time.

% \subsection{Efficiency of Twin Quantization Format}
\label{efficiency_twin_quantization}
Matrix multiplication is a basic operation, which can be well supported by different hardware devices including CPU and GPU.
We can slightly modify the code of matrix multiplication to support the proposed data format for twin uniform quantization.

% \begin{minipage}[t]{0.9\linewidth} 
\begin{lstlisting}[caption=Modification of the innermost loop for 8-bit matrix multiplication,label=twin_format_code]
// Before modification
tmp=A[i][k]*B[k][j];
O[i][j]=O[i][j]+tmp;

// After modification
tmp=(A[i][k]&0x01111111)*B[k][j];
if(A[i][k]&0x10000000)
    tmp=tmp<<m;
// else tmp=-tmp;//Uncomment for post-GELU MatMul
O[i][j]=O[i][j]+tmp;
\end{lstlisting}
% \end{minipage}

The innermost loop of the matrix multiplication code is the multiply-add operation.
The modification is demonstrated in \cref{twin_format_code}.
Firstly, we execute bitwise-and to get the lower $k$-1 bits.
Then, if the MSB of A[i][k] is 1, we left shift the multiplication result by $m$ bits to align the scaling factor.
The alignment is simple because we constraint $\Delta_{\text{R2}}=2^{m}\Delta_{\text{R1}}$.
In this way, we can efficiently process the custom data format on CPU and GPU without extra multiplication and extra data movement.
We evaluate the overhead of the modified matrix multiplication.
Compared with the normal version, the latency on CPU is 1.38x and the latency on GPU is 1.07x.
Moreover, there is potential to further increase the efficiency by designing a specific hardware accelerator.
% \footnote{CPU is Intel Xeon E5-2698 v4 @ 2.2GHz (single thread). GPU is Nvidia Tesla V100-DGX (32G). The size of A is 577x577 and the size of B is 577x1280. The format of A is 8-bit twin quantization format and B is 8-bit signed integer.}.

% \subsection{Number of Calibration Images}

% \begin{table}[]
% \caption{Comparing with the time of quantization and the Top-1 accuracy under different number of calibration images with one Nvidia Tesla V100 GPU. T means the quantization time measured in minutes. }
% \label{QuantTime}
% % \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}ccccccc@{}}
% \toprule
% \multirow{2}{*}{Model} & \multicolumn{3}{c}{\#ims=32} & \multicolumn{3}{c}{\#ims=128} \\
%                       & W8A8      & W6A6     & T     & W8A8      & W6A6      & T     \\ \midrule
% ViT-S/224/32           & 75.58     & 71.91    & 2     & 75.54     & 72.29     & 5     \\
% ViT-S/224              & 81.00     & 78.63    & 3     & 80.99     & 78.44     & 7     \\
% ViT-B/224              & 84.25     & 81.65    & 4     & 84.27     & 81.84     & 13    \\
% ViT-B/384              & 85.83     & 83.35    & 12    & 85.81     & 83.84     & 43    \\ \midrule
% DeiT-S/224             & 79.47     & 76.28    & 3     & 79.41     & 76.51     & 7     \\
% DeiT-B/224             & 81.48     & 80.25    & 4     & 81.54     & 80.30     & 16    \\
% DeiT-B/384             & 82.97     & 81.55    & 14    & 83.01     & 81.67     & 52    \\ \midrule
% Swin-T/224             & 81.25     & 80.47    & 3     & 81.27     & 80.30     & 9     \\
% Swin-S/224             & 83.11     & 82.38    & 8     & 83.15     & 82.38     & 17    \\
% Swin-B/224             & 85.15     & 84.01    & 10    & 85.17     & 84.15     & 23    \\
% Swin-B/384             & 86.39     & 85.39    & 25    & 86.36     & 85.45     & 69    \\ \bottomrule
% \end{tabular}
% % }
% \end{table}

% One of the targets of PTQ4ViT is to quickly quantize a vision transformer.
% In \cref{PTQ4ViT_framework}, we propose to pre-compute the output and gradient of each layer and compute the influence of scaling factor candidates in batches to reduce the quantization time.
% As demonstrated in \cref{QuantTime}, PTQ4ViT can quantize most vision transformers in several minutes using 32 calibration images.
% Using $\#ims=128$ significantly increases the quantization time.
% We observe the Top-1 accuracy varies slightly, demonstrating PTQ4ViT is not very sensitive to $\#ims$. 


